CyLens: Towards Reinventing Cyber Threat Intelligence in the Paradigm of Agentic Large Language Models

The exponential growth of cyber threat knowledge, exemplified by the expansion of databases such as MITRE-CVE and NVD, poses significant challenges for cyber threat analysis. Security professionals are increasingly burdened by the sheer volume and complexity of information, creating an urgent need for effective tools to navigate, synthesize, and act on large-scale data to counter evolving threats proactively. However, conventional threat intelligence tools often fail to scale with the dynamic nature of this data and lack the adaptability to support diverse threat intelligence tasks. In this work, we introduce CYLENS, a cyber threat intelligence copilot powered by large language models (LLMs). CYLENS is designed to assist security professionals throughout the entire threat management lifecycle, supporting threat attribution, contextualization, detection, correlation, prioritization, and remediation. To ensure domain expertise, CYLENS integrates knowledge from 271,570 threat reports into its model parameters and incorporates six specialized NLP modules to enhance reasoning capabilities. Furthermore, CYLENS can be customized to meet the unique needs of different or ganizations, underscoring its adaptability. Through extensive evaluations, we demonstrate that CYLENS consistently outperforms industry-leading LLMs and state-of-the-art cybersecurity agents. By detailing its design, development, and evaluation, this work provides a blueprint for leveraging LLMs to address complex, data-intensive cybersecurity challenges.

==> 04method.tex <==

\section{Fine-Tuning, Inference, and Customization}
\label{sec:ft}

This section details the development of \system after pre-training, focusing on task-oriented dataset construction for fine-tuning (\cref{ssec:ft}), modularized inference (\cref{ssec:inference}), and organizational customization (\cref{ssec:custom}).


\subsection{Fine-Tuning with Cascading Reasoning}
\label{ssec:ft}

{\bf Data Construction.} CTI analysis follows a {\bf cascading} process, which starts with an initial set of evidence and progressively gathers additional information to refine the analysis \cite{oosthoek2021cyber,saeed2023systematic}. To equip LLMs with cascading analytical capabilities, we design the fine-tuning dataset to reflect progressive CTI activities: \(D = \{ E_0 \cup (Q_i, A_i)_{i=1}^n \}\) where \(E_0\) represents the initial evidence, and each query-answer pair \((Q_i, A_i)\) corresponds to a step in the cascading reasoning process: 
\[
(A_1|E_0, Q_1) \rightarrow (A_2 | E_0, A_1, Q_2) \rightarrow ... \rightarrow (A_n | E_0, A_1, ..., A_{n-1}, Q_n)
\]
% \begin{example}
% A \((Q_i, A_i)\) pair requesting identification of a threat actor could be structured as follows:  \\
% \fbox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{
% \label{example:qa}
% \( \mathbf{Q_i} \): \textbf{Evidence:} Logs from the Online Travel Agency (OTA) v.1.0 show multiple POST requests to {\small \texttt{user\_edit.php}} with unusual SQL payloads in the {\small \texttt{user\_id}} parameter, such as: {\small \texttt{POST /user\_edit.php HTTP/1.1  Host: ...}}

% \textbf{Question:} Who is responsible for the unauthorized data deletions and access anomalies occurring on the platform?

% \( \mathbf{A_i} \): The question seeks to identify the threat actor, who is an external attacker exploiting an SQL injection vulnerability in the Online Travel Agency by injecting malicious SQL code through the  {\small \texttt{user\_id}}  in  {\small \texttt{user\_edit.php.}}
% }}
% \end{example}

\begin{example}
Below is a cascading reasoning example.\\
\fbox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{
\label{example:cascading}
\( \mathbf{E_0} \): A security monitoring system detected suspicious outbound traffic from several workstations within the organization’s network. Traffic analysis indicates command-and-control (C2) communication with IP addresses known to be associated with APT28, with observed indicators of $\cdots$ \\
{\bf Step 1: Threat Actor Attribution} \\
\(\mathbf{Q_1}\): From above, what threat actor is likely responsible? \\
\(\mathbf{A_1}\): The observed indicators —including C2 domain, malware characteristics, and past attack patterns— suggest that the activity is associated to APT28, a {\color{black!40}{\shadowtext{XXXX}}} -sponsored threat group known for cyber espionage. \\
{\bf Step 2: Vulnerability Identification} \\
\(\mathbf{Q_2}\): What known vulnerabilities (CVEs) are commonly associated with APT28 in recent campaigns? \\
\(\mathbf{A_2}\): APT28 has exploited CVE-2023-12345 (Windows Kernel Privilege Escalation) and CVE-2023-67890 (Remote Code Execution via malicious DLL sideloading). \\
{\bf Step 3: Prioritization of Threat Response} 
$\cdots$
}}
\end{example}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/figure2.pdf}
    % \includegraphics[width =155mm]{figures/nlp_module.pdf}
    \caption{An illustration of modularization in \system, using the same threat report as described in Example \ref{example:cascading}.}
    \label{fig:nlp-module}
\end{figure*}


Table \ref{tab:ft-data} presents the analytical targets for CTI tasks \ding{182}-\ding{187}, where each task builds upon the preceding ones. As illustrated in Example \ref{example:cascading}, identifying CVEs requires first pinpointing threat actors, which subsequently guides the prioritization.

To construct the fine-tuning dataset, we aggregate references from MITRE-CVE, NVD, and ATT\&CK. For each reference, we extract available evidence as listed in Table \ref{tab:ft-data} and utilize descriptive reports as the initial evidence set \(E_0\). We then generate \((Q_i, A_i)\) pairs following the format exemplified in Example \ref{example:cascading}. It is important to note that not all constructed data samples encompass the full pipeline of tasks \ding{182}-\ding{187}. Detailed dataset statistics are provided in Appendix \ref{app:ft}. 

{\bf Fine-Tuning.} To enable \system with cascading reasoning capabilities, we fine-tune it using the dataset \(D\) described above. The fine-tuning process follows a standard instruction-tuning objective \cite{xu2023lemur,ji2024sevenllm}, where the model is trained to generate a sequence of answers conditioned on the preceding context. Let \(\theta\) represent the parameters of \system. The objective function is defined as:  
\begin{equation}
\begin{split}
  \mathcal{L}(\theta) = - \mathbb{E}_{(E_0, Q_{1\sim n}, A_{1\sim n}) \in D}\ell(E_0, Q_{1\sim n}, A_{1\sim n}, \theta) \\ \text{s.t.}\quad \ell =\sum_{i=1}^{n} \log P_\theta(A_i | E_0, A_1, \dots, A_{i-1}, Q_i)  
\end{split}
\end{equation}
where \( P_\theta(A_i | E_0, A_1, \dots, A_{i-1}, Q_i) \) represents the probability assigned by the model to the correct response \(A_i\) given the accumulated context up to step \(i\).


\begin{table*}[!t]
  \small
  \def\arraystretch{0.95}
  \setlength{\tabcolsep}{4pt}
  \caption{Evaluation results for \ding{182} {\bf Attribution} tasks, where "Hist."--historical threats, "0-Day"--zero-day threats. All metrics are scaled to 0-100 (\%) for consistency. The {\bf boldface} and \underline{underline} highlight the best and second-best results, respectively.}
  \begin{center}
  \scalebox{0.94}{
  % \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
  \begin{tabular}{ccccccccccccccccc}
    \toprule
     & \multicolumn{4}{c}{\bf Threat Actor} & \multicolumn{8}{c}{\bf TTP} & \multicolumn{4}{c}{\bf Campaign} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-13} \cmidrule(lr){14-17}
    % \cline{2-15}
     {\bf Model} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{BERT Score} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall} & \multicolumn{2}{c}{F1 Score} & \multicolumn{2}{c}{IoU} & \multicolumn{2}{c}{Accuracy} & \multicolumn{2}{c}{BERT Score} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
    % \cline{2-15}
    & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day & Hist. & \hlcell 0-Day \\
    % \toprule
    \midrule
    % \hline
    % \hline
    \sevenllm & 65.94 & \hlcell 61.17 & 81.25 & \hlcell 79.83 & 73.44 & \hlcell 68.62 & 76.85 & \hlcell 71.53 & 75.11 & \hlcell 70.04 & 60.14 & \hlcell 53.90 & 73.56 & \hlcell 78.42 & 82.19 & \hlcell 80.65 \\
    \lily & 63.62 & \hlcell 54.58 & 78.25 & \hlcell 75.27 & 64.71 & \hlcell 55.32 & 70.17 & \hlcell 64.62 & 59.65 & \hlcell 67.28 & 42.50 & \hlcell 50.69 & 76.25 & \hlcell 70.38 & 82.16 & \hlcell 82.43 \\
    % SOTA3 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 & 00.00 & \hlcell 00.00 \\
    \midrule
    % \hline
    \gpt & 48.33 & \hlcell 40.31 & 76.02 & \hlcell 73.63 & 74.46 & \hlcell 77.42 & 81.53 & \hlcell 80.52 & 77.83 & \hlcell 78.94 & 63.71 & \hlcell 65.21 & 67.76 & \hlcell 69.74 & 76.15 & \hlcell 79.90 \\
    \gpto & 57.36 & \hlcell 55.34 & 77.93 & \hlcell 78.69 & 81.26 & \hlcell 72.49 & 83.18 & \hlcell 82.90 & 82.21 & \hlcell 77.35 & 69.79 & \hlcell 63.06 & 78.82 & \hlcell 72.78 & 77.22 & \hlcell 78.06 \\
    \gemini & 61.06 & \hlcell 57.43 & 81.24 & \hlcell 78.63 & 78.11 & \hlcell 79.36 & 81.19 & \hlcell 82.24 & 79.62 & \hlcell 80.77 & 66.14 & \hlcell 67.75 & 62.82 & \hlcell 69.21 & 75.84 & \hlcell 74.43 \\
    \llama & 34.85 & \hlcell 24.62 & 74.20 & \hlcell 71.35 & 72.46 & \hlcell 60.29 & 78.93 & \hlcell 71.08 & 75.56 & \hlcell 65.24 & 60.72 & \hlcell 48.41 & 41.64 & \hlcell 25.72 & 74.54 & \hlcell 71.58 \\
    \deepseek & 57.85 & \hlcell 55.26 & 80.39 & \hlcell 79.92 & 73.24 & \hlcell 71.51 & 76.43 & \hlcell 79.85 & 74.80 & \hlcell 75.45 & 59.75 & \hlcell 60.58 & 65.71 & \hlcell 63.04 & 78.27 & \hlcell 77.91 \\
    \claude & 30.12 & \hlcell 22.64 & 73.51 & \hlcell 72.96 & 69.82 & \hlcell 54.84 & 77.95 & \hlcell 75.26 & 73.66 & \hlcell 63.45 & 58.30 & \hlcell 46.46 & 58.91 & \hlcell 52.64 & 76.46 & \hlcell 72.83 \\
    \midrule
    % \hline
    \systems-1B & 82.81 & \hlcell 79.52 & 83.84 & \hlcell 81.72 & 86.15 & \hlcell 83.22 & 85.72 & \hlcell \underline{87.44} & 85.93 & \hlcell 85.28 & 75.34 & \hlcell 74.33 & 85.28 & \hlcell 80.61 & 84.62 & \hlcell 81.55 \\
    \systems-8B & \underline{87.58} & \hlcell \underline{83.74} & \underline{86.72} & \hlcell {\bf 85.39} & {\bf 90.67} & \hlcell {\bf 88.70} & {\bf 93.75} & \hlcell {\bf 92.74} & {\bf 92.18} & \hlcell {\bf 90.68} & {\bf 85.50} & \hlcell {\bf 82.94} & {\bf 95.71} & \hlcell {\bf 87.79} & {\bf 88.45} & \hlcell \underline{85.21} \\
    \systems-70B & {\bf 96.53} & \hlcell {\bf 88.29} & {\bf 87.93} & \hlcell \underline{84.52} & \underline{89.63} & \hlcell \underline{87.57} & \underline{88.26} & \hlcell 85.46 & \underline{88.94} & \hlcell \underline{86.50} & \underline{80.08} & \hlcell \underline{76.21} & \underline{91.53} & \hlcell \underline{86.06} & \underline{87.32} & \hlcell {\bf 87.03} \\
    \bottomrule
    % \hline
  \end{tabular}
  }
  \end{center}
\label{tab:expt-1}
\end{table*}


\subsection{Modularized Inference}
\label{ssec:inference}

At each reasoning step \((E_0, A_1, \dots, A_{i-1}, Q_i) \rightarrow A_i\) during inference, we employ various NLP techniques to modularize the analytical process. Table \ref{tab:ft-data} summarizes the NLP techniques used for each task. These techniques are implemented through the following approaches:

{\bf Topic Modeling.} We implement topic modeling to interpret users' intentions regarding the tasks they aim to perform. Specifically, we use \texttt{BERTopic}, a transformer-based package that eliminates the need for manually setting hyperparameters, as required in conventional methods \cite{blei2003latent, lee2000algorithms}. Given a threat report \(E_0\), we implement a two-step approach: first, based on CTI tasks \ding{182}-\ding{187}, and then, based on specific analytical targets, as outlined in Table \ref{tab:ft-data}.

\begin{example} Topic modeling (Figure \ref{fig:nlp-module}-(b)).\\
\fbox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{
Using the same example as in \ref{example:cascading}, the topic modeling step first determines the task as {\bf threat attribution} based on {\bf $Q_1$}. It then further specifies the analytical target as the {\bf threat actor} within the threat attribution task.}}
\end{example}

{\bf Named Entity Recognition (NER) and Relation Extraction.} Next, we extract entities relevant to the identified topics while simultaneously identifying relationships among them. We employ the multi-agent generation approach described in \cref{ssec:pt-data}, utilizing few-shot prompting, where task-specific entities and their relationships are included as demonstrations within the prompt. This approach facilitates a structured understanding of cybersecurity threats, enhancing the accuracy and contextual relevance of extracted threat intelligence.


{\bf Retrieval Augmented Generation (RAG).} We implement RAG to retrieve relevant web documents through web screening to enrich threat reports. This is especially useful for zero- 
\begin{example}
NER and relation extraction (Figure \ref{fig:nlp-module}-(c)). \\
\fbox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{
Using Example \ref{example:cascading}, the NER identifies key entities {\bf "APT28"} and {\bf "C2 communication"} within the threat report. Simultaneously, relation extraction determines the {\bf "is associated with"} relationship between these entities. }}
\end{example}
day threat hunting, where web-scale CTI intelligence—such as reported threat groups, affected products, and potential patches—is continuously updated. Then, we prompt GPT-o1 to rank the retrieved documents based on their relevance to the threat report $E_0$. To {\bf control latency}, we implement a cache to store retrieved documents. Caching documents are indexed by topic modeling results (i.e., CTI tasks and analytical targets) and specific entities (e.g., APT28 or C2 communication). 

{\bf Reasoning and Summarization.} We implement reasoning and summarization through prompting in \system, where reasoning is applied when deeper analysis or multi-step thinking is required. For example, reasoning is used to analyze severity level (e.g., medium) based on gathered evidence. Summarization is then applied to synthesize insights, tailoring the output to a specific CTI task by leveraging results from topic modeling, NER, relation extraction, and RAG.
% Detailed prompt designs are provided in \cref{app:nlp}. 

{\bf Cascading Reasoning in Inference.} Since CTI tasks exhibit dependencies (Table \ref{tab:ft-data}), we minimize latency by concurrently executing topic modeling, NER, relation extraction, and RAG across all prerequisite tasks. Reasoning and summarization then proceed sequentially, following task dependencies to generate structured, step-by-step findings and conclusions.

% \begin{example}
% Using the same evidence as in Example \ref{example:qa}, but with a new question:  ``How can we remediate the SQL injection in the Online Travel Agency v.1.0?'' We have:  

% \(\mathbf{ C_i} \) (CoT regarding threat attribution):   
% ``The SQL injection  is caused by an external attacker exploiting ...''

% \( \mathbf{ A_i} \):  ``To remediate the SQL injection: (1) Web Application Firewall (WAF) – Deploy a WAF to detect and block malicious SQL payloads targeting vulnerable endpoints such as {\small \texttt{customer\_edit.php}}... (2) Least Privilege...'' 
% \end{example}



% \subsection{Fine-Tuning with Retrieving}
% \label{ssec:ft}

% In addition to enhancing \system's CoT reasoning, fine-tuning also aims to integrate Retrieval-Augmented Generation (RAG), enabling \system to analyze zero-day threats more effectively by leveraging the latest CTI knowledge.

% RAG typically employs a transformer-like retriever, which has a significantly smaller parameter scale compared to LLMs. Thus, the retriever requires substantially less tuning effort. To address this, we propose two distinct fine-tuning strategies:

% {\bf Fine-Tuning.}  
% As illustrated in Figure \ref{fig:ft}(a), we begin by independently fine-tuning the LLM, \(\theta\), using the CoT-augmented dataset \(D = \{(Q_i, C_i, A_i)\}_{i=1}^n\), formulating as:
% \begin{equation}
% \theta^* = \arg \min_{\theta} \sum_{i=1}^{n} \ell\left(\theta(Q_i, C_i), A_i\right)
% \label{eq:llm-loss}
% \end{equation}
% The loss $\ell(\cdot, \cdot)$ is designed to enhance the model's reasoning by incorporating CoT processes. As a result, the fine-tuned LLM is more likely to generate outputs with CoT reasoning.


% {\bf Joint Fine-Tuning.} As illustrated in Figure \ref{fig:ft}(b), after \(\theta\) undergoes independent fine-tuning for several epochs, we proceed to fine-tune it concurrently with a retriever, \(\psi\), to align their parameters within the same functional space. To achieve this, we augment the dataset \(D\) with relevant threat corpus entries derived from \cref{ssec:pt-data}, denoted as \(d_i\) (consistent with \cref{ssec:pt}). This results in an updated dataset \(D = \{(Q_i, C_i, A_i, d_i)\}_{i=1}^n\). The corresponding model updating is formulated as:
% \begin{equation}
% \theta^*, \psi^* =  \arg \min_{\theta, \psi} \ell_\texttt{RAG} = \arg \min_{\theta, \psi} (\ell_\theta + \lambda \cdot \ell_\psi) 
% \end{equation}
% where the loss objective \(\ell_\theta = \sum_{i=1}^{n} \ell\left(\theta(Q_i, C_i, d_i), A_i\right)\) is used to fine-tune \(\theta\) with the augmented dataset, ensuring the model generates responses aligned with the target answers \(A_i\). Similarly, \(\ell_\psi = \sum_{i=1}^{n}\sum_{j=1}^{m} \texttt{sim}(d_{ij}, A_i)\) represents the loss objective for fine-tuning the retriever \(\psi\), optimizing it over the chunked corpus \(d_{ij}\) using the embedding similarity function \(\texttt{sim}(\cdot, \cdot)\). The objectives \(\ell_\theta\) and \(\ell_\psi\) are balanced by a scalar \(\lambda\) to harmonize the training of both the LLM and the retriever.

% Overall, as illustrated in Figure \ref{fig:ft}, we iteratively alternate between independent and joint fine-tuning to update \(\theta\) and \(\psi\), ensuring their functional alignment in RAG. The selected hyperparameters are detailed in Table \ref{tab:stat}.

% \subsection{\system Inference}


% The inference process of \system is depicted as follows:  

% \begin{mitemize}
%      \item [\textbf{1.}] \(\mathbf{\psi: Q_i \rightarrow d_i}\) – The retriever \(\psi\) extracts a relevant set of corpus \(d_i\) using the query \(Q_i\). 
%      \item [\textbf{2.}] \(\mathbf{\theta: (Q_i, d_i) \rightarrow C_i}\) – The LLM \(\theta\) generates CoT evidence \(C_i\) based on the RAG-enriched information \((Q_i, d_i)\).  
%     \item [\textbf{3.}] \(\mathbf{\theta: (Q_i, C_i, d_i) \rightarrow A_i}\) – The LLM \(\theta\) leverages the enriched query \((Q_i, C_i, d_i)\) to generate the final answer \(A_i\). 
% \end{mitemize}

% In zero-day threat hunting, LLMs can produce hallucinations when autonomously crawling online information. To mitigate this, we proactively collect and preprocess data from public databases (e.g., MITRE-CVE and Exploit-DB), constructing a curated corpus for reliable retrieval.  

% {\bf Latency Control.} To address the latency introduced by RAG, we retrieve only the ``summary'' of threat reports (as exemplified in \ref{}). Additionally, we implement a cache to store embedded summaries for future retrieval, reducing redundant computations. Notably, CoT reasoning does not introduce significant inference latency, as the generation of both \(C_i\) and \(A_i\) can be completed sequentially within a single execution. 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width =80mm]{figures/ft.pdf}
%     \caption{Fine-tuning workflow of \system.}
%     \label{fig:ft}
% \end{figure}


\subsection{Organizational Customization}
\label{ssec:custom}

Although \system is developed using massive CTI knowledge, it also enables customization to meet specific organizational interests on particular threat categories, specific products, or assisting an entire organization. Such customization is achieved by further fine-tuning LLMs but specifying the scope of data—for example, concentrating on cyber threats related to a single organization. This targeted customization enhances the relevance of CTI in meeting organizational needs.

We demonstrate \system's potential for tailored customization in \cref{ssec:expt-custom}. Through experiments, we highlight its adaptability and flexibility in addressing diverse CTI challenges across different organizational settings.



